Quantum-optical sensing and target detection

This thesis presents three studies in quantum-enhanced sensing and target detection. The first study explores covert target detection using optical or microwave probes, establishing quantum-mechanical limits on the error probabilities of entanglement-assisted detection methods while maintaining the sender's covertness. It identifies the minimal energy required to preserve covertness and reduce error probabilities, compares two-mode squeezed vacuum probes and coherent states against these limits, and extends the analysis to discriminating thermal loss channels and non-adversarial quantum illumination. The second study focuses on phase-insensitive optical amplifiers, determining the quantum limit on the precision of gain estimation using multimode probes possibly entangled with ancillary systems. It finds that the average photon number and the number of input modes are interchangeable resources for achieving optimal gain sensing precision, contrasting classical probes with quantum probes and highlighting the advantages of the latter, even with single-photon inputs and inefficient photodetection. It also provides a closed-form expression for the energy-constrained Bures distance between two amplifier channels. The third study compares three probe states -- coherent state, two-mode squeezed vacuum (TMSV), and single-photon entangled state (SPES) -- in quantum-enhanced target detection, assessing their performance under signal energy constraints relevant to covert radar sensing. SPES is uniquely positioned as a practical probe due to its non-classical properties after thermal loss and ease of generation. Numerical analysis shows that at low signal energies, the error exponent of TMSV aligns with SPES, indicating comparable detection capabilities and that SPES surpasses the best classical state-the coherent state-in accuracy for certain signal strengths.

==> Intro/abstract.tex <==
\theabstract{
\noindent
This thesis encompasses three pivotal studies in the realm of quantum-enhanced sensing and target detection, each addressing unique aspects of quantum optics and information.

The first study delves into covert target detection using optical or microwave probes. It establishes quantum-mechanical limits on the error probability performance of entanglement-assisted target detection, ensuring the sender's covertness from an adversary. This research outlines the minimum energy requirement for maintaining covertness while achieving significant error probability reduction. It compares the efficacy of two-mode squeezed vacuum probes and Gaussian-distributed coherent states against these limits and also extends to quantum limits in discriminating thermal loss channels and non-adversarial quantum illumination.

The second study focuses on phase-insensitive optical amplifiers, fundamental in both theoretical and practical applications. It identifies the quantum limit of precision in estimating the gain of such amplifiers using multimode probes, possibly entangled with an ancillary system. Remarkably, it finds the average photon number $N$ and the number of input modes $M$ to be interchangeable resources for optimal gain sensing. The study compares classical probes with quantum probes, highlighting the advantages of the latter, even with single-photon probes and in cases of inefficient photodetection. It also presents a closed-form expression for the energy-constrained Bures distance between two amplifier channels.

The third study compares three different probe states - coherent state, two-mode squeezed vacuum (TMSV), and single-photon entangled state (SPES) - in quantum-enhanced target detection. It characterizes their performance under signal energy constraints, relevant in applications like covert radar sensing. The study uniquely positions SPES as a feasible physical probe for its non-classical properties post thermal loss channel and ease of generation. Through numerical analysis, it demonstrates that for low signal energy, the error exponent of TMSV aligns with SPES, suggesting comparable target detection capabilities. Moreover, SPES shows superior accuracy over the best classical state, the coherent state, for certain signal strengths.

Collectively, these studies contribute to the development of a comprehensive understanding of quantum sensing limits and the efficacy of various quantum probe states, paving the way for advancements in quantum metrology and related applications.
}
\keywords{
quantum information;
quantum illumination;
quantum metrology;
quantum sensing;
quantum optics;
quantum channel discrimination;
hypothesis testing}


==> Intro/acknowledgement/acknowledgements.tex <==
\acknowledgements
{
As I stand at the culmination of this incredible journey towards earning my PhD, I am filled with immense gratitude towards those who have been pillars of support, guidance, and inspiration throughout this challenging but rewarding journey.

First and foremost, I extend my heartfelt thanks to my supervisor, Assoc. Prof. Mile, for his invaluable guidance, encouragement, and advice. The countless hours spent in discussion and debate have not only sharpened my understanding but also significantly heightened my interest in our field of research. His insights and expertise have been a beacon of light in navigating the complexities of my PhD studies.

I am especially grateful to my unofficial co-supervisor, Dr. Ranjith, for his close mentorship and advanced knowledge sharing. His inspiring ideas and motivations have been instrumental in shaping my doctoral journey. The numerous occasions we spent discussing, debating, and brainstorming ideas have been pivotal in my academic growth.

My sincere appreciation goes to my friend XiMing Wang. His studious nature and companionship during those late nights in the office have been a source of motivation. His assistance with various mathematical concepts has been invaluable.

I would also like to express my gratitude to my colleagues and friends - Ho Matthew, WenYu Guo, MinJeong Song, and Jianjun Chen. Their initiative in organizing weekly badminton sessions on Sundays provided essential relaxation and joy, greatly enriching my PhD experience and alleviating monotony. I also appreciate the thought-provoking discussions with $\textsc{Y}^2$.

A special mention to RuoCheng Huang for the unforgettable conference trip to Lisbon, Portugal. His efforts in planning the itinerary transformed the trip into a fun and fascinating experience, creating memories that I will always cherish.

Gratitude is also due to Eng Swee Gan and Zhan Fei Yeo for making my PhD journey more enjoyable and interesting. To Eng Swee, I am thankful for the unwavering support and motivation, and for providing additional computing equipment that eased my computational tasks. To Zhan Fei, I appreciate the moments we shared having meals and lightening the mood with jokes, offering each other much-needed respite during our arduous PhD journey. His mathematical suggestions were always helpful.

Lastly, but most importantly, I extend my deepest gratitude to my family - my father, mother, and brother, for their constant support and encouragement. Their belief in me has been a source of strength. A special thanks to my greatest supporter, my fiancée Hui Fang Koh, for her unwavering support and companionship. The four-year journey of pursuing a PhD seemed daunting and endless, but with her by my side, it was a journey made easier and much more enjoyable.

To all of you, I am eternally grateful. Thank you for being part of my PhD journey.
}


==> Intro/acknowledgement/declaration.tex <==
\declaration{

%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter*{Candidate Statement of Originality}
I hereby certify that the work embodied in this thesis is the result of original research, is free of plagiarised materials, and has not been submitted for a higher degree to any other University or Institution. I confirm that the investigations were conducted in accord with the ethics policies and integrity standards of Nanyang Technological University and that the research data are presented honestly and without prejudice.
\vspace{4cm}

\noindent
\begin{tabular*}{\textwidth}{%
  @{\extracolsep{\fill}}
  w{l}{3cm}
  c
  w{l}{6cm}
  @{}
}
% \today 
&& \\
\cmidrule(r){1-1}\cmidrule(l){3-3}
Date && Guo Yao Tham
\end{tabular*}

% %%%%%%%%%%%%%%%%%%%%%%%%%
\chapter*{Supervisor declaration}

I have reviewed the content and presentation style of this thesis and declare it is of sufficient quality and grammatical clarity to be examined.  To the best of my knowledge, it is free of plagiarism and the research and writing are those of the candidate except as acknowledged in the Author Attribution Statement. To the best of my knowledge, the investigations were conducted in accord with the ethics policies and integrity standards of Nanyang Technological University and that the research data are presented honestly and without prejudice.
\vspace{4cm}

\noindent
\begin{tabular*}{\textwidth}{%
  @{\extracolsep{\fill}}
  w{l}{3cm}
  c
  w{l}{6cm}
  @{}
}
% \today 
&& \\
\cmidrule(r){1-1}\cmidrule(l){3-3}
Date && Assoc. Prof. Mile Gu
\end{tabular*}




% %%%%%%%%%%%%%%%%%%%%%%%%%
\chapter*{Authorship Attribution Statement}

This thesis contains material from the following 2 papers and 1 poster where I was listed as an author.
\begin{itemize}
\setlength\itemsep{-0.5em}
\item 1 published journal article
\item 1 journal article under review
\item 1 conference poster
\end{itemize}
% Please amend the statements below to suit your circumstances if (B) is selected. Include all papers that are submitted, published, and in preparation.


% %%%%%%%%%%%%%%%%%%%%%%%%%%% MAIN PAPERS
% \vspace{.2cm}
\subsubsection*{Chapter 3:}
Chapter 3 is a journal article under review:

\noindent \textbf{Tham G.Y.}, Nair R., Gu M., (2023) Quantum limits of covert target detection \textit{Phys. Rev. Lett.}, Under review.

 \noindent The contributions of the co-authors are as follows:
    \begin{itemize}
    \setlength\itemsep{-0.45em}
    \item Assoc. Prof. Gu and Dr. Nair provided the initial project direction.
    \item I prepared the manuscript drafts, which were later edited by Dr. Nair and revised by Assoc. Prof. Gu.  
    \item Dr. Nair and I carried out the principle research, encompassing establishing the theoretical setup, derivation of analytical bound, and numerical analysis.
    \item I developed all the \textsc{Matlab} codes for numerical calculations and simulations.
    \item All authors contributed to the research conception, discussion and final manuscript preparation.
    \end{itemize}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{.2cm}
\subsubsection*{Chapter 4:}
Chapter 4 is a journal article published as:

\noindent \textbf{Nair R.}, Tham G.Y., Gu M., (2022) Optimal Gain Sensing of Quantum-Limited Phase-Insensitive Amplifiers \textit{Phys. Rev. Lett. 128, 180506}

\noindent The contributions of the co-authors are as follows:
    \begin{itemize}
    \setlength\itemsep{-0.45em}
    \item Dr. Nair carried out the principle research, including analytical proofs and numerical results.
    \item I assisted in the partial derivation of analytical proofs, and development of \textsc{Matlab} codes for the generation of some numerical results. 
    \item Dr. Nair prepared the manuscript drafts, which were later edited by myself and revised by Assoc. Prof. Gu.
    \item All authors contributed to the research conception, discussion and final manuscript preparation.
    \end{itemize}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{.2cm}
\subsubsection*{Chapter 5:}
Chapter 5 is a conference poster presented as follows.

\noindent \textbf{Tham G.Y.}, Nair R., Gu M., (2022) Single-photon entangled states for quantum-optimal target detection \textit{International Conference on Quantum Communication, Measurement and Computing (QCMC)}

\noindent The contributions of the co-authors are as follows:
    \begin{itemize}
    \setlength\itemsep{-0.45em}
    \item Assoc. Prof. Gu and Dr. Nair provided the initial project direction.
    \item Dr. Nair and I carried out the principle research, encompassing derivation of analytical bound, and numerical analysis.
    \item All authors contributed to the research conception, discussion and final poster preparation.
    \end{itemize}
\noindent We the undersigned agree with the above stated “proportion of work undertaken” for each of the above published (or submitted) peer-reviewed manuscripts contributing to the thesis:

\vspace{.5cm}
\noindent Signed:
\vspace{1cm}

\noindent 
\parbox[b]{0.4\linewidth}{% size of the first signature box
    \strut \\~\\
    \hrule
    \vspace{0.5cm}
    Guo Yao Tham \\
    Student\\
    School of Physical and Mathematical Sciences \\
    Nanyang Technological University \\
    Date: } 
\hspace{1cm} % distance between the two signature blocks % do not add par here
\parbox[b]{0.4\linewidth}{% ...and the second one
    \strut \\~\\
    \hrule
    \vspace{0.5cm}
    Assoc. Prof. Mile Gu \\
    Supervisor \\
    School of Physical and Mathematical Sciences \\
    Nanyang Technological University \\
    Date: } 
    % \par\vspace{1cm} 
    
\vspace{1.5cm}
\noindent 
\parbox[b]{0.4\linewidth}{% size of the first signature box
    \strut \\~\\
    \hrule
    \vspace{0.5cm}
    Dr. Ranjith Nair \\
    Co-supervisor \\
    School of Physical and Mathematical Sciences \\
    Nanyang Technological University \\
    Date: } 


}
